Classification vs. Regression in Supervised Learning for Single Channel Speaker Count Estimation

The task of estimating the maximum number of concurrent speakers from single channel mixtures is important for various audio-based applications, such as blind source separation, speaker diarisation, audio surveillance or auditory scene classification. Building upon powerful machine learning methodology, we develop a Deep Neural Network (DNN) that estimates a speaker count. While DNNs efficiently map input representations to output targets, it remains unclear how to best handle the network output to infer integer source count estimates, as a discrete count estimate can either be tackled as a regression or a classification problem. In this paper, we investigate this important design decision and also address complementary parameter choices such as the input representation. We evaluate a state-of-the-art DNN audio model based on a Bi-directional Long Short-Term Memory network architecture for speaker count estimations. Through experimental evaluations aimed at identifying the best overall strategy for the task and show results for five seconds speech segments in mixtures of up to ten speakers.

==> figures/confusion.tex <==
% This file was created by matplotlib2tikz v0.6.14.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.927647058823529,0.927647058823529,0.949019607843137}

\begin{axis}[
xlabel={$k$},
ylabel={$\hat{k}$},
xmin=0, xmax=11,
ymin=0, ymax=11,
xtick={0.5,1.5,2.5,3.5,4.5,5.5,6.5,7.5,8.5,9.5,10.5},
xticklabels={0,1,2,3,4,5,6,7,8,9,10},
ytick={0.5,1.5,2.5,3.5,4.5,5.5,6.5,7.5,8.5,9.5,10.5},
yticklabels={0,1,2,3,4,5,6,7,8,9,10},
tick align=outside,
tick pos=left,
width=1\textwidth,
height=1\textwidth,
font=\fontsize{11}{12}\selectfont,
x grid style={white},
y grid style={white},
axis line style={white},
axis background/.style={fill=color0},
colorbar,
colormap={mymap}{[1pt]
  rgb(0pt)=(0.968627450980392,0.988235294117647,0.992156862745098);
  rgb(1pt)=(0.898039215686275,0.96078431372549,0.976470588235294);
  rgb(2pt)=(0.8,0.925490196078431,0.901960784313726);
  rgb(3pt)=(0.6,0.847058823529412,0.788235294117647);
  rgb(4pt)=(0.4,0.76078431372549,0.643137254901961);
  rgb(5pt)=(0.254901960784314,0.682352941176471,0.462745098039216);
  rgb(6pt)=(0.137254901960784,0.545098039215686,0.270588235294118);
  rgb(7pt)=(0,0.427450980392157,0.172549019607843);
  rgb(8pt)=(0,0.266666666666667,0.105882352941176)
},
point meta min=0,
point meta max=1,
colorbar style={width=4pt, axis line style={draw=none}, ytick={0,0.2,0.4,0.6,0.8,1},yticklabels={0.0,0.2,0.4,0.6,0.8,1.0},ylabel={}}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=0, xmax=11, ymin=0, ymax=11] {figures/confusion_matrix.png};

\end{axis}

\end{tikzpicture}


==> figures/duration.tex <==
% This file was created by matplotlib2tikz v0.6.13.
\begin{tikzpicture}

\definecolor{color1}{rgb}{0.298039215686275,0.447058823529412,0.690196078431373}
\definecolor{color0}{rgb}{0.927647058823529,0.927647058823529,0.949019607843137}

\begin{axis}[
xlabel={Duration \(D\) in Frames},
ylabel={MAE},
xmin=-0.5, xmax=8.5,
ymin=0.135857456148673, ymax=0.786816272987562,
xtick={0,1,2,3,4,5,6,7,8},
xticklabels={100,200,300,400,500,600,700,800,900},
ytick={0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8},
yticklabels={0.0,0.2,0.3,0.4,0.5,0.6,0.7,},
tick align=outside,
tick pos=left,
x grid style={white},
xmajorgrids,
ymajorgrids,
y grid style={white},
axis line style={white},
axis background/.style={fill=color0},
width=\textwidth,
height=0.6\textwidth
]
\addplot [only marks, draw=color1, fill=color1, colormap/blackwhite]
table{%
x                      y
+0.000000000000000e+00 +6.385012990646495e-01
+1.000000000000000e+00 +4.156636288682126e-01
+2.000000000000000e+00 +3.866786050449682e-01
+3.000000000000000e+00 +3.366750172732503e-01
+4.000000000000000e+00 +2.637021331951673e-01
+5.000000000000000e+00 +2.624647418728959e-01
+6.000000000000000e+00 +2.581671791258833e-01
+7.000000000000000e+00 +2.647957418016120e-01
+8.000000000000000e+00 +2.645404355185759e-01
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
0 0.638501299064649
1 0.415663628868213
2 0.386678605044968
3 0.33667501727325
4 0.263702133195167
5 0.262464741872896
6 0.258167179125883
7 0.264795741801612
8 0.264540435518576
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
0 0.529501745070873
0 0.757227235858521
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
1 0.331229177698919
1 0.50777318536896
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
2 0.302866441412883
2 0.470527138303221
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
3 0.256214672080081
3 0.416434186077932
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
4 0.205581195002823
4 0.323809986137185
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
5 0.190651073067454
5 0.334762156170043
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
6 0.181574955025837
6 0.352612918248687
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
7 0.165446493277713
7 0.367320912424733
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
8 0.18797697232341
8 0.343365533924186
};
% \path [draw=black, fill opacity=0] (axis cs:500,0.135857456148673)
% --(axis cs:500,0.786816272987562);
%
% \path [draw=white, fill opacity=0] (axis cs:1,0.135857456148673)
% --(axis cs:1,0.786816272987562);
%
% \path [draw=white, fill opacity=0] (axis cs:-0.5,0)
% --(axis cs:8.5,0);
%
% \path [draw=white, fill opacity=0] (axis cs:-0.5,1)
% --(axis cs:8.5,1);

\end{axis}

\end{tikzpicture}


==> figures/src-mae-feature.tex <==
% This file was created by matplotlib2tikz v0.6.13.
\begin{tikzpicture}

\definecolor{color1}{rgb}{0,0.447058823529412,0.698039215686274}
\definecolor{color0}{rgb}{0.927647058823529,0.927647058823529,0.927647058823529}
\definecolor{color3}{rgb}{0.835294117647059,0.368627450980392,0}
\definecolor{color2}{rgb}{0,0.619607843137255,0.450980392156863}
\definecolor{color4}{rgb}{0.8,0.474509803921569,0.654901960784314}


\begin{axis}[
xlabel={$k$},
ylabel={MAE},
xmin=-0.5, xmax=10.5,
ymin=-0.0772346843650762, ymax=1.27547568471466,
xtick={0,1,2,3,4,5,6,7,8,9,10},
xticklabels={0,1,2,3,4,5,6,7,8,9,10},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2,1.4},
yticklabels={0.0,0.0,0.2,0.4,0.6,0.8,1.0,1.2,},
tick align=outside,
tick pos=left,
x grid style={white},
ymajorgrids,
xmajorgrids,
width=\textwidth,
height=0.9\textwidth,
y grid style={white},
axis line style={white},
axis background/.style={fill=color0},
legend style={{font=\fontsize{7}{8}\selectfont}, at={(0.03,0.97)}, anchor=north west, draw=none, fill=color0},
legend cell align={left},
legend entries={{MEL40},{MFCC20},{STFT},{STFTLOG}},
]
\addplot [only marks, draw=color1, fill=color1, colormap/blackwhite]
table{%
x                      y
-5.000000000000000e-02 +0.000000000000000e+00
+9.500000000000000e-01 +4.933420704265813e-02
+1.950000000000000e+00 +2.204995712876628e-01
+2.950000000000000e+00 +3.788771103375745e-01
+3.950000000000000e+00 +5.094745938989440e-01
+4.950000000000000e+00 +6.511281488701961e-01
+5.950000000000000e+00 +7.334710815502373e-01
+6.950000000000000e+00 +8.051378526783228e-01
+7.950000000000000e+00 +8.011811009542211e-01
+8.949999999999999e+00 +8.143658785038659e-01
+9.949999999999999e+00 +9.071969720048936e-01
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
-0.05 0
0.95 0.0493342070426581
1.95 0.220499571287663
2.95 0.378877110337575
3.95 0.509474593898944
4.95 0.651128148870196
5.95 0.733471081550237
6.95 0.805137852678323
7.95 0.801181100954221
8.95 0.814365878503866
9.95 0.907196972004894
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
-0.05 0
-0.05 0
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
0.95 0.0255348177253875
0.95 0.0796878426936913
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
1.95 0.169891257357241
1.95 0.269616714828069
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
2.95 0.31468394176693
2.95 0.448208677717223
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
3.95 0.431734496167669
3.95 0.619745913671585
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
4.95 0.538516391462318
4.95 0.815948297769123
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
5.95 0.610192840694834
5.95 0.86939280335924
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
6.95 0.687969929147932
6.95 0.931302230999982
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
7.95 0.710192477046035
7.95 0.901607611985292
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
8.95 0.678013464906467
8.95 0.982716045421449
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
9.95 0.594470750517917
9.95 1.23772622229977
};
\addplot [only marks, draw=color2, fill=color2, colormap/blackwhite]
table{%
x                      y
-1.666666666666667e-02 +0.000000000000000e+00
+9.833333333333333e-01 +3.318052821770502e-02
+1.983333333333333e+00 +1.627906959930645e-01
+2.983333333333333e+00 +2.872006293835245e-01
+3.983333333333333e+00 +4.000861291018773e-01
+4.983333333333333e+00 +5.721583698038448e-01
+5.983333333333333e+00 +6.657483943894547e-01
+6.983333333333333e+00 +7.504177047694437e-01
+7.983333333333333e+00 +6.942257231406131e-01
+8.983333333333333e+00 +5.842873207112621e-01
+9.983333333333333e+00 +4.313973045911050e-01
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
-0.0166666666666667 0
0.983333333333333 0.033180528217705
1.98333333333333 0.162790695993065
2.98333333333333 0.287200629383525
3.98333333333333 0.400086129101877
4.98333333333333 0.572158369803845
5.98333333333333 0.665748394389455
6.98333333333333 0.750417704769444
7.98333333333333 0.694225723140613
8.98333333333333 0.584287320711262
9.98333333333333 0.431397304591105
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
-0.0166666666666667 0
-0.0166666666666667 0
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
0.983333333333333 0.0176544422399854
0.983333333333333 0.0517354284887664
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
1.98333333333333 0.119939706790278
1.98333333333333 0.213393619020921
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
2.98333333333333 0.24457204693034
2.98333333333333 0.337666866377517
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
3.98333333333333 0.333758609516676
3.98333333333333 0.465127037912222
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
4.98333333333333 0.519359312023493
4.98333333333333 0.632827803652405
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
5.98333333333333 0.548789027724603
5.98333333333333 0.771814738880395
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
6.98333333333333 0.68901420088614
6.98333333333333 0.827730780956938
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
7.98333333333333 0.625967855918387
7.98333333333333 0.771872264099872
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
8.98333333333333 0.516049388406587
8.98333333333333 0.671391695267557
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
9.98333333333333 0.308059764284678
9.98333333333333 0.543386986074022
};

\addplot [only marks, draw=color3, fill=color3, colormap/blackwhite]
table{%
x                      y
+1.666666666666666e-02 +1.068376068774070e-03
+1.016666666666667e+00 +1.178781938954824e-02
+2.016666666666667e+00 +1.307062879268924e-01
+3.016666666666667e+00 +2.638398129646573e-01
+4.016666666666667e+00 +3.548664931435712e-01
+5.016666666666667e+00 +4.763729270213003e-01
+6.016666666666667e+00 +5.445362752572017e-01
+7.016666666666667e+00 +6.263575650994342e-01
+8.016666666666667e+00 +6.170166188546262e-01
+9.016666666666667e+00 +6.473625136010441e-01
+1.001666666666667e+01 +6.632996624969072e-01
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
0.0166666666666667 0.00106837606877407
1.01666666666667 0.0117878193895482
2.01666666666667 0.130706287926892
3.01666666666667 0.263839812964657
4.01666666666667 0.354866493143571
5.01666666666667 0.4763729270213
6.01666666666667 0.544536275257202
7.01666666666667 0.626357565099434
8.01666666666667 0.617016618854626
9.01666666666667 0.647362513601044
10.0166666666667 0.663299662496907
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
0.0166666666666667 0.000213675213874214
0.0166666666666667 0.00192307692387293
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
1.01666666666667 0.00742196035877619
1.01666666666667 0.0165902644174179
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
2.01666666666667 0.103138457616016
2.01666666666667 0.157412791026886
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
3.01666666666667 0.226732429847689
3.01666666666667 0.300942286036245
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
4.01666666666667 0.325355296669902
4.01666666666667 0.379414295554033
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
5.01666666666667 0.40547573544361
5.01666666666667 0.544082590648662
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
6.01666666666667 0.501825070798507
6.01666666666667 0.588842979237725
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
7.01666666666667 0.562447790618528
7.01666666666667 0.691765875866638
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
8.01666666666667 0.551175626361464
8.01666666666667 0.699278211609272
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
9.01666666666667 0.528597081632392
9.01666666666667 0.773540965222851
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
10.0166666666667 0.469460226404747
10.0166666666667 0.902598903792274
};
\addplot [only marks, draw=color4, fill=color4, colormap/blackwhite]
table{%
x                      y
+5.000000000000000e-02 +2.564102577833602e-03
+1.050000000000000e+00 +1.440733485747209e-02
+2.050000000000000e+00 +1.397502149144809e-01
+3.050000000000000e+00 +2.917157429594782e-01
+4.050000000000000e+00 +4.173126569038625e-01
+5.050000000000000e+00 +5.376756059687002e-01
+6.050000000000000e+00 +6.664370988026138e-01
+7.050000000000000e+00 +7.389306559000995e-01
+8.050000000000001e+00 +6.736657949048808e-01
+9.050000000000001e+00 +6.435465781375616e-01
+1.005000000000000e+01 +5.505050503043614e-01
};
\addplot [line width=1.00pt, color4, forget plot]
table {%
0.05 0.0025641025778336
1.05 0.0144073348574721
2.05 0.139750214914481
3.05 0.291715742959478
4.05 0.417312656903862
5.05 0.5376756059687
6.05 0.666437098802614
7.05 0.7389306559001
8.05 0.673665794904881
9.05 0.643546578137562
10.05 0.550505050304361
};
\addplot [line width=1.00pt, color4, forget plot]
table {%
0.05 0.000854700868426918
0.05 0.00448717951424854
};
\addplot [line width=1.00pt, color4, forget plot]
table {%
1.05 0.00785854626229684
1.05 0.0240176821835861
};
\addplot [line width=1.00pt, color4, forget plot]
table {%
2.05 0.102912359958086
2.05 0.174644701583287
};
\addplot [line width=1.00pt, color4, forget plot]
table {%
3.05 0.249293286086568
3.05 0.339031209053072
};
\addplot [line width=1.00pt, color4, forget plot]
table {%
4.05 0.377255595644212
4.05 0.462537673636822
};
\addplot [line width=1.00pt, color4, forget plot]
table {%
5.05 0.471237759145905
5.05 0.622844826140179
};
\addplot [line width=1.00pt, color4, forget plot]
table {%
6.05 0.592056937367956
6.05 0.748461892527654
};
\addplot [line width=1.00pt, color4, forget plot]
table {%
7.05 0.659121751329654
7.05 0.836680241890171
};
\addplot [line width=1.00pt, color4, forget plot]
table {%
8.05 0.573889991229079
8.05 0.780900045564481
};
\addplot [line width=1.00pt, color4, forget plot]
table {%
9.05 0.524562289451743
9.05 0.761470258544491
};
\addplot [line width=1.00pt, color4, forget plot]
table {%
10.05 0.382970326311058
10.05 0.708769997357319
};
\end{axis}

\end{tikzpicture}


==> figures/src-mae-objective.tex <==
% This file was created by matplotlib2tikz v0.6.13.
\begin{tikzpicture}

\definecolor{color3}{rgb}{0.9450980392,0.6392156863,0.2509803922}
\definecolor{color0}{rgb}{0.927647058823529,0.927647058823529,0.927647058823529}
\definecolor{color1}{rgb}{0.36862745,  0.23529412,  0.6}
\definecolor{color2}{rgb}{0.59803922,  0.7745098 ,  0.44117647}

\begin{axis}[
xlabel={$k$},
ylabel={MAE},
xmin=-0.5, xmax=10.5,
ymin=-0.0792013957712289, ymax=1.33125716523073,
xtick={0,1,2,3,4,5,6,7,8,9,10},
xticklabels={0,1,2,3,4,5,6,7,8,9,10},
ytick={-0.2,0,0.2,0.4,0.6,0.8,1,1.2,1.4},
yticklabels={0.0,0.0,0.2,0.4,0.6,0.8,1.0,1.2,},
tick align=outside,
tick pos=left,
x grid style={white},
ymajorgrids,
xmajorgrids,
width=\textwidth,
height=0.9\textwidth,
y grid style={white},
axis line style={white},
axis background/.style={fill=color0},
legend style={{font=\fontsize{7}{8}\selectfont}, at={(0.03,0.97)}, anchor=north west, draw=none, fill=color0},
legend entries={{Classification},{Gaussian Regr.},{Poisson Regr.}},
legend cell align={left}
]
\addplot [only marks, draw=color1, fill=color1, colormap/blackwhite]
table{%
x                      y
-3.750000000000001e-02 +6.410256410256410e-04
+9.625000000000000e-01 +2.259332023575639e-02
+1.962500000000000e+00 +1.280684754521964e-01
+2.962500000000000e+00 +2.663427561837455e-01
+3.962500000000000e+00 +3.709625322997416e-01
+4.962500000000000e+00 +5.164431673052363e-01
+5.962500000000000e+00 +5.981404958677685e-01
+6.962500000000000e+00 +7.687969924812030e-01
+7.962500000000000e+00 +8.047900262467192e-01
+8.962500000000000e+00 +8.131313131313130e-01
+9.962500000000000e+00 +4.267676767676769e-01
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
-0.0375 0.000641025641025641
0.9625 0.0225933202357564
1.9625 0.128068475452196
2.9625 0.266342756183746
3.9625 0.370962532299742
4.9625 0.516443167305236
5.9625 0.598140495867769
6.9625 0.768796992481203
7.9625 0.804790026246719
8.9625 0.813131313131313
9.9625 0.426767676767677
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
-0.0375 0
-0.0375 0.0016025641025641
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
0.9625 0.0145628683693517
0.9625 0.0320890635232482
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
1.9625 0.0960876937984496
1.9625 0.164256298449612
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
2.9625 0.2262882803298
2.9625 0.309190959952886
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
3.9625 0.316210432816537
3.9625 0.419101259689923
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
4.9625 0.430707215836526
4.9625 0.600139687100894
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
5.9625 0.501291322314049
5.9625 0.696121728650138
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
6.9625 0.69046835839599
6.9625 0.842575187969925
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
7.9625 0.714554625984252
7.9625 0.891437007874016
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
8.9625 0.722516835016835
8.9625 0.897988215488216
};
\addplot [line width=1.00pt, color1, forget plot]
table {%
9.9625 0.292589962121212
9.9625 0.610483743686869
};
\addplot [only marks, draw=color2, fill=color2, colormap/blackwhite]
table{%
x                      y
+0.000000000000000e+00 +9.615384721352408e-04
+1.000000000000000e+00 +4.780615648875634e-02
+2.000000000000000e+00 +1.889534884442886e-01
+3.000000000000000e+00 +3.303886937598388e-01
+4.000000000000000e+00 +4.691537419954936e-01
+5.000000000000000e+00 +6.198914547761282e-01
+6.000000000000000e+00 +7.358815521001816e-01
+7.000000000000000e+00 +7.742794503768285e-01
+8.000000000000000e+00 +6.369750648736954e-01
+9.000000000000000e+00 +5.127946138381958e-01
+1.000000000000000e+01 +6.071654036641121e-01
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
0 0.000961538472135241
1 0.0478061564887563
2 0.188953488444289
3 0.330388693759839
4 0.469153741995494
5 0.619891454776128
6 0.735881552100182
7 0.774279450376829
8 0.636975064873695
9 0.512794613838196
10 0.607165403664112
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
0 0.000160256410405661
0 0.00192307695397176
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
1 0.0265185005535992
1 0.0736738717610327
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
2 0.153088661360865
2 0.226102230853091
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
3 0.276060073326031
3 0.397232040762901
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
4 0.396455096205076
4 0.575637913805743
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
5 0.521220470344027
5 0.73771154868106
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
6 0.63892045840621
6 0.845742959529161
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
7 0.677001087119182
7 0.89132988974452
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
8 0.573978828266263
8 0.712955214455724
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
9 0.469507576711476
9 0.557596805940072
};
\addplot [line width=1.00pt, color2, forget plot]
table {%
10 0.486576702507834
10 0.74371054880321
};

\addplot [only marks, draw=color3, fill=color3, colormap/blackwhite]
table{%
x                      y
+3.750000000000001e-02 +1.121794871794872e-03
+1.037500000000000e+00 +1.113294040602489e-02
+2.037500000000000e+00 +1.732881136950905e-01
+3.037500000000000e+00 +3.194935217903416e-01
+4.037500000000000e+00 +4.211886304909561e-01
+5.037500000000000e+00 +5.416666666666666e-01
+6.037500000000000e+00 +6.236225895316805e-01
+7.037500000000000e+00 +6.475563909774437e-01
+8.037500000000000e+00 +6.478018372703412e-01
+9.037500000000000e+00 +6.912457912457913e-01
+1.003750000000000e+01 +8.803661616161618e-01
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
0.0375 0.00112179487179487
1.0375 0.0111329404060249
2.0375 0.17328811369509
3.0375 0.319493521790342
4.0375 0.421188630490956
5.0375 0.541666666666667
6.0375 0.62362258953168
7.0375 0.647556390977444
8.0375 0.647801837270341
9.0375 0.691245791245791
10.0375 0.880366161616162
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
0.0375 0
0.0375 0.00272435897435897
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
1.0375 0.00605762933857236
1.0375 0.0173583824492469
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
2.0375 0.135493378552972
2.0375 0.215128391472868
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
3.0375 0.283119846878681
3.0375 0.36588265606596
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
4.0375 0.397771317829457
4.0375 0.443802487080103
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
5.0375 0.514683109833972
5.0375 0.571208492975734
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
6.0375 0.588304924242424
6.0375 0.657558539944904
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
7.0375 0.600716635338346
7.0375 0.692046522556391
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
8.0375 0.596604330708662
8.0375 0.718836122047244
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
9.0375 0.5765867003367
9.0375 0.829124579124579
};
\addplot [line width=1.00pt, color3, forget plot]
table {%
10.0375 0.678484059343434
10.0375 1.1229521780303
};
\end{axis}

\end{tikzpicture}

